Contextual Emotion Estimation from Image Captions

Emotion estimation in images is a challenging task, typically using computer vision methods to directly estimate people's emotions using face, body pose and contextual cues. In this paper, we explore whether Large Language Models (LLMs) can support the contextual emotion estimation task, by first captioning images, then using an LLM for inference. First, we must understand: how well do LLMs perceive human emotions? And which parts of the information enable them to determine emotions? One initial challenge is to construct a caption that describes a person within a scene with information relevant for emotion perception. Towards this goal, we propose a set of natural language descriptors for faces, bodies, interactions, and environments. We use them to manually generate captions and emotion annotations for a subset of 331 images from the EMOTIC dataset. These captions offer an interpretable representation for emotion estimation, towards understanding how elements of a scene affect emotion perception in LLMs and beyond. Secondly, we test the capability of a large language model to infer an emotion from the resulting image captions. We find that GPT-3.5, specifically the text-davinci-003 model, provides surprisingly reasonable emotion predictions consistent with human annotations, but accuracy can depend on the emotion concept. Overall, the results suggest promise in the image captioning and LLM approach.

==> sections/signal_table.tex <==
% \begin{table*}[t]
% \caption{Physical Signals Used to Annotate the Image Captions}
% \begin{center}
% \begin{tabular}{p{3cm}|p{14cm}}
% \hline
% \textbf{Signal Categories}&\textbf{Physical Signals} \\
% \hline
% Eyes Signals & Closed eyes, Frowning, Staring off into the distance, Furrowed eyebrows, Glaring, Side-eyeing, Averted gaze, Looking up, Squeezing eyes shut, Rolling eyes, Avoiding eye contact, Looking away, Lowered eyebrows, Empty stare, Raising eyebrows, Squinting eyes, Looking sideway, Eyebrows squishing together, Eyes wide open, Looking down, Peeking, Eyes are damp and bright, Staring down at the ground, Unfocused gaze, Downcast eyes, Raising one's eyebrows, Gaze clouding, Glassy stare, Refusing to look, Glancing as if looking for answers, Eyes are co, glaring, Side look \\
%  \hline
%  Mouth Signals & Gritting teeth, Open mouth, Mouth wide open, Clenched jaw, Downturned mouth, Biting lips, Lips that flatten, Smiling, Sticking tongue out, Curling lip, Poking one's tongue into the cheek, Yawning, Smirking, Breathing excessively, Biting finger, Pressing lips tight, Grimacing\\
% \hline
% Facial Signals & High chin, Flat expression, Crying, Chin dipping down, Resting one side of face on hand, Resting chin on hand, Tilting one's head to the side, Smelling oneself, Hiding face in arms, Tilting head downward, Leaning head on hand, Using something to hide face, Wrinkling nose, Resting forehead on hand, Puffing out the cheeks, Tilting head upward, Grimacing, Lips that flatten or curl, Wrinkling one's nose, Expression that appears pained\\
% \hline
% Body Signals & Sitting, Bending down, Bent spine, Bending forward, Visible sweating, Leaning back, Hunched shoulders, Leaning forward, Body posture that loosens or collapses, Lying flat, Bracing against a wall, Chest caving, Bending forward and laying head on arms, Shoulders slumping or curling forward, Leaning on an object, Falling onto ground, Tight shoulders, Naked body, Tense posture, Picking fights, Body freezing in place, Turning body away, Curling up body into a ball, Stiff posture, Slouching on an object, Hood over the head, Throwing up, Covering oneself with something, Keeping one's back to a wall, Sliding down in a chair, Slouching and leaning on objects, Visible tension in the neck, Hands covering face, Pointing fingers, Pulling a hood over the head, Rubbing the affected area of one's body \\
% \hline
% Hands Signals & Hand up in air, Folding arms across the chest, Hand wiping tears, Covering face with hands, Thumbs down, Pressing a fist to the mouth, Throwing things, Pointing middle finger, Palms open, Curling fingers, Rubbing one's forehead or eyebrows, Hands in pockets, Cheek resting on own palm, Crossed arms, Squeezing nose, Grabbing onto someone, Hand on own chest, Hand resting on forehead, Hands on both sides of head, Rubbing the eyes, Grabbing own hair, Clenched fists, Pointing finger, Scratching at cheek or temple, Rubbing the foot, Arms reaching out, Gripping something and knuckles going white, Palms covering forehead, Palms up facing outward, Hands on the hip, Rubbing temples, Rubbing the back of the neck, Hands covering ears, Rubbing the back, Taking off eyeglasses, Hand on neck, Throwing hands up in the air, Wiping tears, Rubbing the shoulder, Sweeping hand across the forehead to get rid of sweat, Clapping palms together, Hand covering mouth, Rubbing the chest, Hands curling around their body, Rubbing the nose, Clutching the stomach, Hand touching the lips, Nervous hand gestures \\
% \hline
% Feet Signals & Knees pulling together, Bringing the feet together, Squatting \\
% \hline

% \hline
% % \multicolumn{3}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
% \end{tabular}
% \label{signal_table}
% \end{center}
% \end{table*}




\begin{table*}
% \begin{longtable}{p{3cm}|p{14cm}}
\caption{Other Contextual Information Used to Annotate the Image Captions}

\begin{tabular}{p{3cm}|p{14cm}}
\hline
\textbf{Signal Categories}&\textbf{Signals} \\
% \endhead
\hline
Environmental & in a office with a computer on a desk, in an office with a laptop and a big pile of folders and documents on the table, on a street, on a couch in a living room, in a waiting room, on a field, at a Formula 1 game, right in front of an alien hand in the dark, in a gym, someone reach out their hand to pinch Greg's face, in a classroom, in the middle of a match, presenting at a meeting, in a meeting, surrounded by many people, in a protest, in a hospital bed giving birth, in a hospital room, on a street on a windy night, in a room with a cellphone on the table, in an office, surrounded by masked people with knives, in a meeting at an office, in a meeting with document on the table, in a living room, in a bathroom stall, beside a window with sunlight, walking on totem poles with friends, at a live show, in an evacuation, on a stage in front of a microphone with flag in the back, on a patio, in a room with friends, in a park, in a stairway, surrounded by a group of people, surrounded by a group of people pointing and laughing at him, has wind blowing, in a office with a laptop on a desk, on a pavement with a helmet and water bottle scattered on the ground, on the side of road with a water bottle and phone scattered around, in a bedroom, in a forest, in a movie theatre, in a garden, on stage in a classroom, in a dark room, at a funeral, in a library with a laptop and a book on the desk, at a party, at a public gathering, at a physiotherapy, in a soccer game and has been given a yellow card, listening to music on a street on a rainy day, in the dark, in a bed, in a living room with a laptop and document on a table, on a couch with a laptop and many documents on the table, at a restaurant with newspaper in hands, in front of a computer, on a couch in a room, at talent show, eating in a movie theatre, in an Olympic game, on a bus, on a steet, on a running track, holding a plate of pancake, in an office with a laptop on a table, in a living room on a couch, in a room with empty chairs, in front of a tombstone at an American cemetery, on a couch, in a boxing match, in the middle of a boxing match, on a bench in a park, in a committee meeting, in a hospital hallway, at a public memorial, on the side of the road and surrounded by another bicyclers, in front of a computer in an office, in a restaurant, in a kitchen, cake falling down at wedding, holding an umbrella on a street, in a soccer game, on a trail that splits into two directions, surrounded by other people, on a phone call, on a subway train, in a dark room watching TV, in a dark bedroom watching TV, in a library, on a bed in a bedroom, at a meeting, surrounded by women crying on the street on a snowy day, on the street on a snowy day, at a table in a living room, in a bathroom, in the shower in a bathroom, on a trail, in a room with a phone on the table, behind window blinds, on a cloudy day at a beach, in an office with a computer on the desk, in an office with documents on the table, at a modelling competition, in a hospital bed with an arm cast, in a crowd gathering and surrounded by people crying, surrounded by people crying, stuck in an iceberg crack, at a social gathering with other people, on a street with a dog jumping and biting, in a room with books, by a beach, at an office, on a grass field, in a dark wooden house, in a suitcase, in a the snow, at an office with documents on the table, wearing a Korean flag ripping apart a Japanese flag and surrounded by cops, at an office with a big pile of documents on the table, given a red card in a soccer game, on a street walking by with a group of people, in a room with a big pile of homework on the table, in a hospital, in a waiting room at a clinic, in the waiting area inside a hospital, on a soccer field, in a corner of a room, holding a pizza, in a room, on a bench in a street, been given a broccoli, having lunch at a theme park, on a ben, holding a snapped phone, in a car, in a jail, biting a pencil and looking at a document, in a clinic, at an office desk, in a school hallway, in the middle of a race, outside a fence, in a parking lot, on a staircase, at s desk with a big pile of documents on it, at a wedding, on a bed, in an office with a laptop on the table, in an office with a laptop on the desk, in a soccer game and the referee calling stop, at a movie theatre, in a hospital bed, on the bathroom floor in the of a toilet, a bowl salad on the table, in a match, camping in a forest with a black bear comping to the camp site, in a cardboard box, at a restaurant, at a sports game, in a tennis match, in a car and a camel is sticking its head into the car window, at a funeral in front of a casket, outdoor, at a table with an empty plate, on an airplane with trays and pillows thrown onto the floor due to turbulence, in a protest with a sign that says Turkey Guilt of Genocide, a dog jumping and biting, on a rope bridge that is falling to one side, looking at phone at a convocation, in a kitchen with receipts on a table, on a grass field with a bicycle falling onto the ground, getting a vaccine shot, on the deck by an ocean, an opened fridge and smelling a drink, holding a toast with brown sauce, in front of a microphone, in front of a tombstone,on a bench by a river, a laptop and a big pile of books on the table, a woman falling off from the balcony, in bullfighting and a bull running towards, at a cemetery with flowers at a desk with a laptop , at a desk with a laptop, at a school, on a street next to a parking meter, in public, surrounded by people laughing and pointing, on the edge of a cliff, reading a book on a bench in a park, in the hallway inside a hotel, on the edge of an ice field, waitress over-pouring coffee and it's spilled on the table, on an airplane, in a tunnel, at a party with cake on the table, a car running into a group of bicyclers on a street, dinner time and someone is feeding him, on a tennis court with a tennis racket on the ground, at teeth cleaning, by a window, on a bed with medication on the side, in front of a laptop, in an elevator filled with smoke, in a soccer game, in a golf match, in a hospital bed and gave birth to a child, on a boat\\

\hline

\end{tabular*}
\end{table}
 
\begin{table*}
% \begin{longtable}{p{3cm}|p{14cm}}
\caption{Other Contextual Information Used to Annotate the Image Captions}

\begin{tabular}{p{3cm}|p{14cm}}
\hline
\textbf{Signal Categories}&\textbf{Signals} \\
% \endhead
\hline
Interaction & Alec is comforting Terry, Jane is putting her hand on Mia's shoulder while Mia has her back turned to Jane, Nancy is following him, clinking glass with Karl, crossing his arms, crying and Nancy is putting her hand on Beth's shoulder, giving birth in a hospital bed and Greg is putting his hand on Beth's head, he is being leaned on by Lucas, he is being yelled at by Chloe and seems annoyed, he is being yelled at by Sophia, he is bleeding and pointing a rifle at Lucas' neck, he is checking Chloe's left leg, he is checking on Jack, he is checking onto Jack, he is clinking glass with Alec, he is covering his ears, he is crying and grabbing onto Jane, he is crying and hugging Wendy, he is discussing with Wendy, he is feeding Chloe a giant pizza, he is frowning and not looking at Chloe, he is giving a presentation, he is giving a thumbs down, he is grabbing onto Terry and carrying him out from the stadium, he is hitting Terry's face, he is hitting his opponent, he is holding Jack in his arms, he is holding onto Sean's body and lifting him up, he is holding up Greg, he is hugged by Chloe but is holding hands with Mia behind her back, he is hugging his partner while holding hands with Wendy behind her back, he is laughing and pointing at Chloe, he is leaning away from Wendy because he is being yelled at by her, he is leaning away from Wendy, seemingly scared, he is looking at Chloe from behind her, he is looking at Sean, he is looking at his phone, he is looking down and being yelled at and pointing at by Greg, he is looking in the opposite direction as Nancy, he is naked and on a bed with Nora, he is peeking at Nancy, he is pointed by Jack with a gun, he is pointing his finger at Wendy, he is pointing his finger at something, he is pulling Greg's tie, he is punching Greg's face, he is putting a hand on Jack's shoulder, he is putting an oxygen mask over Greg's face, he is putting his hand on Terry's head, he is rolling his eyes with hands in the pockets, he is running behind Sophia, he is sitting beside Sophia but turning his body away from her, he is sitting far from Sophia and has turned his back on her, he is sitting next to Sean and putting his hand around Sean's and Alec's shoulder, he is sleeping, he is sleeping beside Nancy, he is sleeping in a seat next to Terry, he is sleeping on Terry's shoulder, he is smiling and pose for camera, he is smiling and thumbs up, he is smiling at his phone and not looking at Chloe, he is staring and smiling at an iPad, he is staring at Chloe and biting his nails, he is talking to someone else, he is throwing his hands in the air and yelling at Sophia, he is trying to calm Jack down, he is yelling and pointing a pen at Sean, he is yelling at Chloe and throwing hands in the air, he is yelling at Jane, he is yelling at Sean, he is yelling at Wendy, her fists and clenched and are in the air, her flowers grew better than Jane's, her hair is being pulled by Chloe, her tie is being pulled by Chloe, his hands are clapped and looking at Sophia, his tie being pulled by Jack, looking at Lucas, on a bed with Lucas, point at Nancy behind her back, pushing a hospital bed, reaching hand out to Nancy, she and Chloe are pulling each other's hair, she has hunched shoulders and resting her chin on her hand while Nancy is putting her hand on Mia's shoulder, she is a seat away from Lucas, reading a magazine, she is also at the accident hugging her son, she is also crossing her arms and has her back to Terry's back, she is also crossing her arms and looking in another direction, she is also crossing her arms and sitting with her back against Jack's back, she is also crying and covering her face with her hands, she is also doing the same thing as Chloe, she is being stared by others, she is being yelled at by Sean, she is bending down and putting her hands on Nancy's back, she is blowing a whistle, she is closing her eyes and covering her ears, she is closing her eyes and covering her face with a hand, she is comforting Chloe by wrapping her arm around Chloe, she is comforting Jane, she is comforting Wendy, she is covering her ears and holding onto Wendy, she is covering her ears with hands and turned her back to Jack, she is crying and being learned onto by Jane, she is crying and grabbing onto Wendy,  she is crying and holding her head with her hands, she is crying and holding onto Jack, she is crying and hugging Chloe, she is eating a lollipop and side-eyed by Chloe, she is following Lucas and her eyes her shut, she is frowning and gritting her teeth at Greg, she is frowning and staring at Terry, she is frowning with her eyes closed, and is being yelled at by Nancy, 
she is gritting her teeth and yelling at Greg, she is holding a bowl of popcorn, she is holding onto Nancy's shoulder, she is holding onto Wendy's hand, she is hugging Chloe and hiding her face, she is hugging Jane, she is kissing Sean, she is laughing and pointing at Greg, she is laughing and pointing at Sophia, she is laughing and pointing finger at Chloe, she is leaning close to Nancy, she is leaning towards Wendy, she is learning toward Chloe looking at Chloe's book, she is looking at Terry, she is looking at her phone, she is looking at the screen and wiping tears, she is looking in the direction where Sean is throwing a wine bottle at, she is naked and taking a shower with Ronald, she is placing her hand on Jack's arm and on a phone call, she is placing her hands on Nancy's stomach, she is pointing a pen at Terry, she is pointing and laughing at Jack, she is pointing and laughing at Sean with others, she is pulling Chloe's hair, she is putting her hand in the air and body turned away from Jack, she is putting her hand onto Chloe's shoulder, she is putting her hand up and looking away from Terry, she is scratching her forehead, she is side-eyeing Jack, she is sitting behind Lucas and kicking Lucas' chair, she is sitting far from Sean crossing her arms and ignoring Sean, she is sitting next to Sophia, she is sitting next to Terry not engaging with him, she is smiling, she is smiling and comforting Chloe, she is smiling and showing her diamond ring to Wendy, she is smiling and talking on the phone, she is taking down notes, she is taking down notes about Lucas, she is turning her back onto Greg , she is wrapping her hand around Lucas, she is yelling at Nancy, she is yelling at Terry, she sleeping with Lucas, she walked into the bathroom and is closing her eyes , sitting next to Jane and reading a magazine, smiling and sitting close to Nora\\
\hline

% \multicolumn{3}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{environment_interaction_table}
\end{table*}


==> trash.tex <==

\section{Ease of Use}

\subsection{Maintaining the Integrity of the Specifications}

The IEEEtran class file is used to format your paper and style the text. All margins, 
column widths, line spaces, and text fonts are prescribed; please do not 
alter them. You may note peculiarities. For example, the head margin
measures proportionately more than is customary. This measurement 
and others are deliberate, using specifications that anticipate your paper 
as one part of the entire proceedings, and not as an independent document. 
Please do not revise any of the current designations.

\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA}--\ref{SCM} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.

%%  ---- START: Added 2022-03-15 for ACII2022 onwards -----
\section*{Ethical Impact Statement}

At ACII2023, we are requiring a {\color{red} mandatory} field to be filled in on the manuscript submission portal to discuss any issues regarding the Ethical Impact of their work. This allows authors to reflect on the ethical impact of the work, which could include societal and environmental impact.

We also {\color{red}highly recommend} authors to include a corresponding Ethical Impact Statement in their papers to discuss these issues. If authors choose to do so, this section should be un-numbered (like the Acknowledgement), and come after the conclusions, but before the Acknowledgement and References. (For example, the text in this section can be used to answer the mandatory field on the manuscript submission portal.)

Please see the Conference Submission Guidelines on the conference website for up-to-date information and guidelines.
%%  ---- END: Added 2022-03-15 for ACII2022 onwards -----

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.

